Resonant mode approximation of the scattering matrix of photonic crystal slabs near several Wood-Rayleigh anomalies

The resonant mode approximation of the scattering matrix is considered for calculating the optical properties of multilayered periodic structures within the formalism of the Fourier-modal method for two diffraction thresholds in close proximity of the spectral-angular range of interest. The developed approximation opens up possibilities for the fast calculation of the scattering matrix of these structures when describing the integral characteristics of spectra and dispersion curves containing high-Q resonances, such as bound states in the continuum.

==> name_deleted.tex <==
It can be easily shown, for example, for} a homogeneous medium, where $\mathcal{E}$ is the identity matrix, and $\mathcal{H}$ consists of four diagonal blocks: % associated with the values of $k_z$:
\begin{gather}
\mathcal{H}
% =\dfrac{c}{\omega\mu}\begin{pmatrix}
% \dfrac{-(k_y+G_y)(k_x+G_x)}{\sqrt{(\frac{\omega}{c})^2\epsilon\mu-(k_x+G_x)^2-(k_y+G_y)^2}}\delta_{\mathbf{GG'}}&\dfrac{-(\frac{\omega}{c})^2\epsilon\mu+(k_x+G_x)^2}{\sqrt{(\frac{\omega}{c})^2\epsilon\mu-(k_x+G_x)^2-(k_y+G_y)^2}}\delta_{\mathbf{GG'}}\\
% \dfrac{(\frac{\omega}{c})^2\epsilon\mu-(k_y+G_y)^2}{\sqrt{(\frac{\omega}{c})^2\epsilon\mu-(k_x+G_x)^2-(k_y+G_y)^2}}\delta_{\mathbf{GG'}}&
% \dfrac{(k_y+G_y)(k_x+G_x)}{\sqrt{(\frac{\omega}{c})^2\epsilon\mu-(k_x+G_x)^2-(k_y+G_y)^2}}\delta_{\mathbf{GG'}}
% \end{pmatrix}=\\
=\dfrac{c}{\omega}\begin{pmatrix}
\dfrac{-K_yK_x}{K_z}& \dfrac{-K_z^2-K_y^2}{K_z}\\
\dfrac{K_z^2+K_x^2}{K_z}&\dfrac{K_yK_x}{K_z}
\end{pmatrix},
\end{gather}
where diagonal matrices $K_{x,y,z}$ are defined as follows:
\begin{align}
    K_x=&\mathrm{diag}\{k_{x}-\frac{2\pi}{d_x}\alpha_x\},\\
    K_y=&\mathrm{diag}\{k_{y}-\frac{2\pi}{d_y}\alpha_y\},\\
    K_z=&\mathrm{diag}\{k^{(\alpha)}_z\},
\end{align}
and $c$ is the speed of light. The expression for the interface matrix connecting the vectors of amplitudes in two adjacent layers reads:
\begin{gather}
\mathbb{I}=\mathbb{F}_{m-1}^{-1}\mathbb{F}_{m}=\{\mathbb{F}_{m-1}\equiv \mathbb{F}\}=\\
=\begin{pmatrix}
\mathbb{F}_{11}^{-1}+\mathbb{F}_{12}^{-1}\mathcal{H}&\mathbb{F}_{11}^{-1}-\mathbb{F}_{12}^{-1}\mathcal{H}\\
\mathbb{F}_{21}^{-1}+\mathbb{F}_{22}^{-1}\mathcal{H}&\mathbb{F}_{21}^{-1}-\mathbb{F}_{22}^{-1}\mathcal{H},
\end{pmatrix}
\end{gather}
with $m$ being the index number of the homogeneous layer where we consider the diffraction threshold. For simplicity of presentation, without loss of generality, we also assume that this is the last layer of the structure; hence, if $\hat{\mathbb{S}}$ is the scattering matrix of the system without the last interface, then the total scattering matrix of the system is \edit{(see Appendix D in \cite{Tikhodeev2002b} for details)}:
%\begin{widetext}
\begin{equation}
\mathbb{S}_\mathrm{tot}=
\begin{pmatrix}
(\mathbb{I}_{11}-\hat{\mathbb{S}}_{12}\mathbb{I}_{21})^{-1}\hat{\mathbb{S}}_{11}& (\mathbb{I}_{11}-\hat{\mathbb{S}}_{12}\mathbb{I}_{21})^{-1}(\hat{\mathbb{S}}_{12} \mathbb{I}_{22}-\mathbb{I}_{12})\\
\hat{\mathbb{S}}_{21}+\hat{\mathbb{S}}_{22}\mathbb{I}_{21}(\mathbb{I}_{11}-\hat{\mathbb{S}}_{12}\mathbb{I}_{21})^{-1}\hat{\mathbb{S}}_{11}& \hat{\mathbb{S}}_{22}(\mathbb{I}_{21}(\mathbb{I}_{11}-\hat{\mathbb{S}}_{12}\mathbb{I}_{21})^{-1}(\hat{\mathbb{S}}_{12}\mathbb{I}_{22}-\mathbb{I}_{12})+\mathbb{I}_{22})
\end{pmatrix}
\label{Sfull}
\end{equation}
